Long-Term Memory-Guided Enhancement for Target Perception in Audio-Language Models

Audio large language models (ALLMs) can reason about the content of audio recordings to perform complex tasks. However, these capabilities usually collapse in real-world environments when background noise and competing sources mix the target sound. Inspired by long-term memory in human listening, we propose Long-Term Memory-Guided Audio Enhancement (LTM-AE) to improve selective target perception by refining the audio representations of ALLMs without training. LTM-AE extracts representations in hidden states from separate clean reference recordings as long-term memory for each category, guiding enhancement toward a user-specified listening target. We reconstruct incoming audio tokens in the selected category long-term memory and interpolate the reconstructions with the original tokens before language backbone decoding. This interpolation controls the influence of stored auditory experience while keeping all ALLM parameters fixed. Diagnostic readouts across twenty sound categories and three ALLMs show that LTM-AE strengthens responses to a specified target amid three interfering sources. Averaged over constrained and free-form classification, accuracy gains over raw mixtures range from 29.53 to 46.15 percentage points across multiple open source models. For speech content recovery, LTM-AE with an additional learned token-level gate reduces Qwen2-Audio's word error rate from 23.07% to 14.77%. This work takes an initial step toward using principles of human long-term memory to enhance ALLMs for real-world listening. Our code is available at https://github.com/aynlp/ltm-audio-code

==> Papers/Papers/0_Abstract.tex <==
\begin{abstract}
Audio large language models (ALLMs) can reason about the content of audio recordings to perform complex tasks.
However, these capabilities usually collapse in real-world environments when background noise and competing sources mix the target sound.
Inspired by long-term memory in human listening~\citep{weinberger2004specific}, we propose Long-Term Memory-Guided Audio Enhancement (LTM-AE) to improve target perception by refining the audio representations of ALLMs without training.
LTM-AE extract representations in hidden states from clean audio input as long-term memory for category, assisting recognize specific audio channels.
We reconstruct incoming audio tokens in the selected category memory and interpolate the reconstructions with the original tokens before language backbone decoding.
This interpolation controls the influence of stored auditory experience while keeping all ALLM parameters fixed.
Experiments on twenty sound categories across three ALLMs show that LTM-AE improves recognition under strong acoustic interference when the target category is known.
With twenty clean examples per category, Qwen2-Audio's constrained classification accuracy increases from 9.60\% on raw mixtures to 47.20\% with LTM-AE at $-10$\,dB.
This work takes an initial step toward using principles of human long-term memory to enhance ALLMs for real-world listening.
Our code is available at \href{https://github.com/xxx/LTM-AE}{\textcolor{cornflowerblue}{LTM-AE}}
\end{abstract}


==> Papers/Papers/1_Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Audio large language models (ALLMs) bridge text and audio inputs, enabling language models to handle complex involving tasks the audio modality~\citep{chu2024qwen2audio, kimiteam2025kimi, stepaudio2025technical}.
Real-world use brings ALLMs into diverse and changing acoustic environments that may differ quite from their training stage.
In these environments, background noise and competing sources mix even overwhelm the target audio channel.
A model that can reason about clean audio may then fail to perceive the same target within a mixture.
Human listening suggests that prior auditory experience can help address this gap between capability and perception under interference~\citep{agus2010rapid}.
Learning recurring sound structure also helps listeners distinguish individual sources within mixtures~\citep{munte2001superior, woods2018schema}.
These findings motivate drawing on methods to guide perception when the current input is obscured.

Audio enhancement has long addressed interference through statistical signal estimation and learned signal reconstruction~\citep{ephraim1984speech, luo2019convtasnet}.
Text descriptions are proven to guide waveform separation by specifying the sound to recover from a mixture~\citep{kilgour2022text, liu2024audiosep, ma2024clapsep}.
For ALLMs, \citet{zhang2026rsabench} have highlighted environmental interference as a major challenge, showing that competing sources can substantially impair both perception and reasoning.
In response, recent methods enhance ALLM perception by recovering a target speaker's speech~\citep{chen2026avdialog, godiva2026noise} or selecting between speech and non-speech components~\citep{yin2026focus}.
Denoising improves ALLM robustness to added noise, with the clean recording defining the content to preserve~\citep{xiong2025thinking, zhang2026see}.
However, ALLMs still struggle to perceive a specified target when multiple stronger sources compete in the same audio, especially when the target is a non-speech sound.
ALLMs have to overcome these perceptual limitations to enable broader applications in real-world scenarios such as embodied intelligence and robotics.

We propose Long-Term Memory-Guided Audio Enhancement (LTM-AE) for enhancing target perception through category memory without training the ALLM.
The memory retains category structure from clean audio, while the current recording determines how that structure enters the reconstruction of each audio token.
To build this memory, we extract hidden states at the interface between the audio pathway and the language backbone.
We store their mean and dominant directions of variation for reuse across later inputs.
At inference, the target category selects the memory, and the incoming tokens determine their reconstruction coefficients within it.
Interpolation with the original tokens then controls the strength of the memory's influence on the current audio representation.
Because reconstruction may discard useful target detail, we calibrate the interpolation weight together with the number of retained directions.
The calibration minimizes token reconstruction error on paired clean and mixed validation recordings, tying the enhancement to its ability to approximate clean target representations.
The resulting tokens retain their original temporal positions for decoding by the language backbone, and all ALLM parameters remain fixed.

We evaluate LTM-AE on mixtures spanning twenty target categories using three ALLMs, with classification and feature retrieval as measures of target perception.
Each test target is mixed with three interfering sources at $-10$\,dB relative to their combined energy.
Without enhancement, Qwen2-Audio identifies the designated target in 9.60\% of constrained classification trials.
The classification prompts ask generically about the main sound, while LTM-AE additionally uses the true target category to select its memory.
Under this oracle protocol, LTM-AE achieves 47.20\% accuracy with category memory constructed from $N=20$ clean recordings per category.
Table~\ref{tab:twenty_class_main} shows that the gains extend to the other backbones and also appear in free-form classification.
Feature retrieval against a clean reference gallery also improves, showing that the effect is present in the audio representations before language backbone decoding.
These gains establish better recognition with the appropriate category memory, while recovery of details specific to the current recording requires further evidence.

We make the following contributions toward enhancing ALLMs for real-world listening.
\begin{itemize}
    \item We introduce LTM-AE as an enhancement method inspired by human long-term memory.
    It combines category memory extracted from clean audio hidden states with the current recording through calibrated reconstruction and interpolation, without training the ALLM.
    \item Across three ALLMs, we demonstrate gains in target recognition under strong interference over twenty sound categories when the target category is known.
    Classification and feature retrieval reveal the effect of the enhancement in both language outputs and audio representations.
\end{itemize}


==> Papers/Papers/2_Related_Works.tex <==
\section{Related Works}

==> Papers/Papers/3_Methods.tex <==
\section{Long-Term Memory-Guided Audio Enhancement}
\label{sec:method}

We use a persistent auditory memory to constrain the audio representations that enter a frozen audio large language model (ALLM).
We build this memory from clean examples of a sound category, whose tokens define an affine subspace in the model's input representation.
When the model receives a new recording, we reconstruct its audio tokens within that subspace and blend the reconstruction with the original sequence.
The stored memory thus guides subsequent inputs without updating the backbone.
This fixed-memory procedure requires no parameter training; the token-wise
gate introduced in Section~\ref{sec:memory_gate} is a separate optional
extension that trains only its lightweight control parameters.

\subsection{Audio Representations and Memory Conditioning}
\label{sec:memory_setting}

Let $F_{\theta}$ denote the pretrained audio pathway from the encoder to the language model's input space.
For an audio input $x$, it produces $Z=F_{\theta}(x)=(z_1,\ldots,z_T)$, where each token $z_t\in\mathbb{R}^{d}$ occupies a temporal position in the sequence.
We modify these tokens before they enter the language model.
The modified sequence occupies the original audio positions, so its length and order remain unchanged alongside the usual text embeddings and attention mask.

The representation at this boundary depends on how the backbone connects audio to language.
Qwen2-Audio supplies the audio encoder's projected outputs~\citep{chu2024qwen2audio}, whereas Kimi-Audio combines discrete audio embeddings with projected continuous features~\citep{kimiteam2025kimi}.
Step-Audio-2-mini supplies the audio adapter outputs~\citep{stepaudio2025technical}.
We fit a separate memory in each model's representation space, allowing the same reconstruction rule to operate at different feature dimensions.

The reconstruction is conditioned on a target category $c$ through its memory $\mathcal{M}_c$.
Our implementation uses the known target category to select this memory.
This oracle selection lets us probe perception conditioned on the appropriate auditory prior.
The mechanism therefore takes $c$ as an input and does not include an automatic selector for an unknown mixture.

\subsection{Constructing a Persistent Auditory Memory}
\label{sec:memory_construction}

For category $c$, we extract audio tokens from $N$ clean reference clips with the frozen pathway.
We stack every valid token into $X_c\in\mathbb{R}^{M_c\times d}$, where $M_c$ is the total token count.
Each row contributes equally to the fit, so clips contribute in proportion to their token counts.
We apply no temporal pooling or individual token normalization before decomposition.
This construction lets one memory capture variation across examples and temporal positions.

We represent that variation through the mean and leading principal directions of the reference tokens~\citep{jolliffe2016principal}.
Writing $\widetilde X_c$ for the centered token matrix, we construct
\begin{equation}
\mu_c=\frac{1}{M_c}\sum_{i=1}^{M_c}X_{c,i}^{\top},\qquad
\widetilde X_c=X_c-\mathbf{1}\mu_c^{\top},\qquad
\mathcal{M}_c=(\mu_c,U_c),
\label{eq:memory}
\end{equation}
where $X_{c,i}$ denotes row $i$ and the columns of $U_c$ are leading right singular vectors of $\widetilde X_c$.
Our default construction obtains them with a randomized low-rank PCA solver~\citep{halko2011finding}.
These orthonormal directions define a subspace around the category mean.
We save the mean and basis for subsequent reconstruction, with singular values and construction metadata available in the memory archive.

The reference count determines which observations support the estimate, while the retained rank determines how much variation the memory can represent.
Once fitted, the memory remains fixed across new recordings.
An incoming mixture can therefore be reconstructed against the clean reference structure without entering the memory fit.

\subsection{Enhancement Through Memory Reconstruction}
\label{sec:memory_enhancement}

For each incoming token, we first subtract the selected category mean and project the centered token onto the retained directions.
Adding the mean back gives a reconstruction in the memory's affine subspace.
We blend this reconstruction with the original token using $\alpha_c\in[0,1]$.
With $U_{c,k}$ containing the first $k$ columns of the stored basis, this yields
\begin{equation}
\begin{aligned}
\widehat z_t&=\mu_c+U_{c,k}U_{c,k}^{\top}(z_t-\mu_c),\\
z'_t&=z_t+\alpha_c(\widehat z_t-z_t).
\end{aligned}
\label{eq:memory_enhancement}
\end{equation}
The resulting sequence replaces the audio embeddings before the language model computes its response.
All temporal positions use the same memory, but each token is reconstructed from its own coordinates along the basis.

To see what this changes, let $P_c=U_{c,k}U_{c,k}^{\top}$ and let $I$ denote the identity matrix.
Separating the centered token into its projection and orthogonal residual gives
\begin{equation}
z'_t=\mu_c+P_c(z_t-\mu_c)
 +(1-\alpha_c)(I-P_c)(z_t-\mu_c).
\label{eq:residual_shrinkage}
\end{equation}
The component within the subspace is unchanged, while the orthogonal residual is multiplied by $1-\alpha_c$.
If a clean target token lies in the affine subspace, reconstruction preserves it and attenuates the orthogonal component of an observed token's error.
This interpretation concerns the geometry of the representations and does not assume that the encoder maps waveform mixtures to additive source embeddings.
Interference within the subspace remains, while useful target variation outside it is attenuated.
Choosing the rank and coefficient therefore requires balancing the retained variation against the strength of the correction.

\subsection{Calibration and Inference Cost}
\label{sec:memory_calibration}

We make this choice with paired clean and mixed audio from a validation partition separate from memory construction.
For each category and reference count, we compare enhanced mixture tokens with their corresponding clean target tokens.
Let $\mathcal{V}_c$ contain these aligned token pairs and let $H_{c,k,\alpha}$ denote Eq.~(\ref{eq:memory_enhancement}).
We select the rank and coefficient by minimizing their reconstruction error:
\begin{equation}
(k_c,\alpha_c)=\underset{(k,\alpha)\in\mathcal{G}}{\operatorname{argmin}}\;
\frac{1}{|\mathcal{V}_c|d}
\sum_{(z,z^{\mathrm{clean}})\in\mathcal{V}_c}
\left\|H_{c,k,\alpha}(z)-z^{\mathrm{clean}}\right\|_2^2,
\label{eq:memory_selection}
\end{equation}
over a predefined finite candidate set $\mathcal{G}$.
The paired validation tokens calibrate the intervention without entering the PCA fit or updating the pretrained parameters.

With calibration complete, inference uses the saved mean and the selected basis columns to apply Eq.~(\ref{eq:memory_enhancement}).
Its two low-rank matrix multiplications cost $O(Tdk)$ arithmetic operations for a sequence of $T$ tokens in $d$ dimensions.
The mean and selected basis require $O(d(k+1))$ storage, even if the offline archive retains additional columns for rank selection.
At fixed $d$ and $k$, increasing the reference count therefore leaves the deployed memory size unchanged.
The audio pathway and language model remain frozen throughout this computation.

\subsection{Optional Token-Wise Control}
\label{sec:memory_gate}

The core LTM-AE procedure above remains training-free and applies a fixed
coefficient across time. As a separate optional extension, we consider a gate
for cases in which fine-grained content may need different correction strengths
at different positions.
For the Qwen speech setting, this gate can reduce the correction at each token.
Let $\delta_t=z'_t-z_t$ be the correction from the calibrated reconstruction.
The gate receives the concatenation of $z_t$ and $\delta_t$, which passes through layer normalization and two linear layers separated by GELU.
A sigmoid converts the network output to a scalar weight:
\begin{equation}
g_t=\sigma\!\left(f_{\phi}([z_t;\delta_t])\right),\qquad
z_t^{\mathrm{gate}}=z_t+g_t\delta_t
 =z_t+g_t\alpha_c(\widehat z_t-z_t).
\label{eq:memory_gate}
\end{equation}
The scalar applies to every feature coordinate at that position.
Because $\delta_t$ already includes $\alpha_c$, the effective reconstruction weight is $g_t\alpha_c$.
The gate thus controls how much of the calibrated correction reaches the language model.

We train this control with a token reconstruction loss and an optional teacher-forced transcription loss:
\begin{equation}
\mathcal{L}(\phi)=
\lambda_{\mathrm{tok}}\operatorname{MSE}(Z^{\mathrm{gate}},Z^{\mathrm{clean}})
 +\lambda_{\mathrm{text}}\mathcal{L}_{\mathrm{CE}}
 (y\mid Z^{\mathrm{gate}}).
\label{eq:gate_objective}
\end{equation}
The first term compares the gated sequence with clean target tokens.
The second uses the reference transcript $y$ to compute cross-entropy through the frozen language model.
Its gradients reach the gate through the modified audio embeddings, so the gate can receive supervision tied to the language output.
Only the gate parameters are updated.
The memory and its calibrated settings stay fixed, as do all ALLM parameters.


==> Papers/Papers/4_Experiments.tex <==
\section{Experiments}

\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:experimental_setup}
We begin with a proof of concept on three sound classes to examine how
clean PCA memories affect representations corrupted by interference.
The subsequent ablations study whether this effect changes with model
adaptation or with the way the memory is constructed. We then extend the
evaluation to twenty sound classes and three ALLMs to examine how the
effect varies across models and categories.

\paragraph{Final20 data and mixture construction.}
For the large-scale evaluation, we assemble Final20, an internal dataset of
twenty sound categories standardized to three-second, 16-kHz, monaural clips.
The source collections are MAESTRO for piano; Dog play/pant, FSD50K, and
UrbanSound8K for dog vocalization; LibriSpeech for human speech; NSynth for
flute and organ; GAPS for classical guitar; the RWC Instruments Database for
violin, trumpet, clarinet, alto saxophone, and drums; CatMeows for cat
vocalization; CowRumIA for cow vocalization; Glass Frog Calls for frog calls;
CrowCall and FSD50K for crow calls; FSD50K for glass breaking and alarms;
FSD50K and UrbanSound8K for car horns; Donate-a-Cry for infant crying; and
DCASE 2013 isolated events together with FSD50K for door slams. Final20 is not
a standalone public benchmark; it is constructed from these source datasets.

For each category, we form three non-overlapping partitions of 100 clips:
\texttt{pca\_train} for memory construction, \texttt{validation} for selecting
$k$ and $\alpha$, and \texttt{mixture\_eval} for final testing. The partitions
are separated by source group, and the construction pipeline applies audio
quality checks and hash-based duplicate removal. The $N\in\{20,50,100\}$
memory conditions use subsets of \texttt{pca\_train}. For every validation or
evaluation target, we select three clean interferers from three distinct
non-target categories. Each interferer is first RMS-matched to the target, and
their sum is then scaled so that the target-to-combined-interference ratio is
$-10$ dB. This yields 2,000 validation mixtures and 2,000 final-evaluation
mixtures. All three ALLMs receive the same final-evaluation audio. A separate
clean reference gallery contains 100 clips per category for retrieval. It
excludes windows that overlap the queries, but recordings from the same source
group may still occur in the gallery and the other partitions.

\paragraph{Audio representation and PCA memory.}
We extract audio tokens or pooled audio representations from each model
and use clean examples to construct a PCA memory for each sound class.
The enhancement moves a mixture's representation toward the principal
subspace of the selected target class. To measure its effect, we compare
the enhanced mixture with the original mixture and the clean target.
Here, $N$ denotes the number of clean examples per class used to construct
the memory, while $k$ denotes the number of retained principal components.

\paragraph{Evaluation protocols.}
In the twenty-class experiment, constrained classification asks the model
to select one of twenty labels. Free-form classification removes these
options and asks for a short sound description. We also evaluate the
representations directly through prompt-free token retrieval. This protocol
compares the audio representation with a separately constructed clean
reference gallery using cosine similarity. We average the five largest
similarities within each class and predict the class with the highest
average, reporting top-one category accuracy. The gallery excludes
overlapping audio windows, although recordings from the same source group
may occur in both the gallery and the other data partitions.

\paragraph{Scope of evaluation.}
In the enhancement experiments, the target label selects the corresponding
PCA memory. The generic prompts ask for the main sound, while scoring checks
the predefined target category, which is weaker than the aggregate
interference. The unenhanced condition does not receive this information
about the target. The comparisons therefore measure target readout
conditioned on a supplied category memory. They do not by themselves
establish recovery of evidence specific to the current audio instance.

\drafttodo{Test dependence on the current audio with a memory-only sequence
of repeated category means, target-absent audio, and wrong-memory controls.
Start with Qwen2-Audio. For one compact matched-cue evaluation, reuse the
existing three-class target-present/absent mixtures and ask whether the cued sound is
present, giving every baseline the same cue. This keeps the answer dependent
on the audio rather than making it identical to the memory label. Report
false positives as well as detection accuracy.}

\subsection{Three-Class Proof-of-Concept}
\label{sec:three_class}
\drafttodo{Link the early three-class study and the following LoRA, local-PCA,
and geometry ablations to their original runs, splits, scoring definitions,
and hyperparameters. Their numerical values are retained from the existing
draft but are not covered by the current Final20 code handoff. Keep them
separate from the frozen-model Final20 evidence until this provenance is checked.}
The initial proof of concept uses three sound
classes from IRMAS: piano, violin, and human voice. The dataset contains
180 clean training examples, with 60 examples per class, and 60 clean test
examples, with 20 examples per class. For each clean test example, we
construct two mixed versions: one mixed with ordinary environmental noise
and one mixed with another sound class. This results in 120 mixed test
examples. The target sound is mixed at $-5$ dB, making it weaker than the
interference.

We extract 4096-dimensional pooled representations with Qwen2-Audio and
build each class's PCA memory from its clean training representations,
retaining at most 32 principal components. We evaluate fixed enhancement
with $\alpha=0.5$ against the unenhanced mixture. A gate that uses
confidence to choose $\alpha\in\{0.2,0.5\}$ provides a second enhancement
condition. To check whether the effect extends beyond the PCA-memory
scoring rule, we also evaluate an independent logistic regression classifier
trained on clean representations.

\begin{table}[t]
\centering
\caption{Accuracy (\%) in the three-class proof-of-concept experiment.
The fixed and gated columns report results after PCA-based representation
enhancement.}
\label{tab:three_class_results}
\small
\begin{tabular}{lcccc}
\toprule
Evaluator & Clean & Mixed & Fixed PCA & Gated PCA \\
\midrule
PCA-memory scorer & 95.0 & 60.0 & 77.5 & -- \\
Logistic regression & 96.7 & 53.3 & 80.0 & 80.8 \\
\bottomrule
\end{tabular}
\end{table}

As shown in Table~\ref{tab:three_class_results}, mixing reduces accuracy
for both evaluators. Fixed PCA enhancement raises the PCA-memory accuracy
from 60.0\% to 77.5\%. It corrects 21 previously misclassified examples
without changing any originally correct example into an incorrect
prediction. The independent logistic regression classifier also improves,
from 53.3\% to 80.0\%, and reaches 80.8\% with gated enhancement. The
improvement therefore extends to a classifier that does not use the
PCA-memory scoring rule, indicating better class separation in the enhanced
representations.

The two forms of interference differ in difficulty. Before enhancement,
the PCA-memory scorer obtains 80.0\% accuracy when the target is mixed with
ordinary noise, but only 40.0\% when it is mixed with another sound class.
This suggests that a competing sound class causes more representation
confusion than ordinary environmental noise in this setting.

\subsection{PCA Design and Ablation Studies}
\label{sec:pca_ablation}
We next examine which design choices affect enhancement. These ablations
use piano, dog vocalization, and guitar as target classes, with evaluation
on the standard test set and a separate generalization set. We begin with
the representation learned by the backbone, then examine how much clean
data and how many principal directions the memory retains. The final
ablation compares global and local memories.

\paragraph{Direct PCA versus LoRA followed by PCA.}
We compare PCA enhancement on the frozen backbone with PCA after LoRA
adaptation, where LoRA uses a masked-token objective on clean audio.
Table~\ref{tab:direct_lora_pca} reports the enhanced classification accuracy.
The two methods are evaluated in their respective representation spaces
and therefore have slightly different clean and mixed baselines.

\begin{table}[t]
\centering
\caption{Classification accuracy (\%) after direct PCA enhancement and
LoRA followed by PCA. ``Gen.'' denotes the generalization set.}
\label{tab:direct_lora_pca}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{Piano}
& \multicolumn{2}{c}{Dog}
& \multicolumn{2}{c}{Guitar} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Method & Test & Gen. & Test & Gen. & Test & Gen. \\
\midrule
Direct PCA & 98 & 98 & 50 & 29 & 8 & 15 \\
LoRA + PCA & 100 & 100 & 69 & 63 & 0 & 0 \\
\bottomrule
\end{tabular}
\end{table}

Direct PCA raises piano test accuracy from the mixed baseline of 38\% to
98\%. It also improves dog recognition from 8\% to 50\%, while the gain for
guitar is limited. LoRA adaptation on clean audio further improves dog
recognition to 69\% on the test set and 63\% on the generalization set, but
reduces the guitar result to 0\%. Thus, adaptation changes the usefulness
of the PCA directions differently across classes.

\paragraph{Effect of clean-memory size.}
With these differences across classes in mind, we vary the number of clean
examples used to construct each memory. Table~\ref{tab:memory_size_ablation}
compares accuracy after enhancement with the clean and mixed baselines.
It also reports the relative reduction in mean squared error (MSE) between
the enhanced and clean audio tokens.

\begin{table}[t]
\centering
\caption{Effect of the number of clean memory examples per class.
All values except $N$ are percentages.}
\label{tab:memory_size_ablation}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccc}
\toprule
Class & $N$ & Clean & Mixed & PCA & MSE reduction \\
\midrule
Piano  & 20  & 100 & 29 & 100 & 42.5 \\
Piano  & 50  & 100 & 30 & 100 & 42.0 \\
Piano  & 100 & 100 & 32 & 100 & 41.7 \\
\midrule
Dog    & 20  & 62 & 2 & 100 & 37.4 \\
Dog    & 50  & 61 & 2 & 98 & 38.2 \\
Dog    & 100 & 62 & 2 & 87 & 37.9 \\
\midrule
Guitar & 20  & 57 & 0 & 1 & 42.9 \\
Guitar & 50  & 56 & 0 & 0 & 42.4 \\
Guitar & 100 & 54 & 0 & 0 & 42.4 \\
\bottomrule
\end{tabular}
\end{table}

Increasing the number of clean examples does not lead to monotonic accuracy
improvements. Piano remains at 100\% for all three memory sizes, whereas
dog accuracy decreases from 100\% at $N=20$ to 87\% at $N=100$. Guitar
remains close to 0\% despite an MSE reduction of more than 42\%. Therefore,
lower token reconstruction error is not sufficient to guarantee better
semantic classification.

\paragraph{Subspace dimensionality and PCA geometry.}
The number of retained directions provides another way to change the
memory's capacity. We compare $k=16$ and $k=128$ principal components.
For the base global PCA memory, increasing $k$ raises the fraction of noise
energy entering the clean subspace from 38.2\% to 69.2\%, while reducing
distortion of the clean representation from 42.1\% to 13.0\%. The reduction
in token MSE nevertheless decreases from 37.7\% to 23.3\%. Similar behavior
occurs after LoRA adaptation. A larger subspace therefore preserves more
clean variation while also admitting more interference.

For guitar, we also examine a PCA memory for each local cluster. This
improves test accuracy from
0\% with global PCA to 11\%, while direct projection onto the clean
subspace reaches 71\%. However, the corresponding routing consistency is
only 34\%. This gap suggests that geometric proximity to a clean
class-specific subspace does not necessarily restore the semantic decision
path used by the audio model.

\subsection{Twenty-Class Cross-Model Evaluation}
\label{sec:twenty_class}
The variation across classes motivates evaluation on a broader set of
twenty sound classes, spanning speech and environmental events as well as
musical instruments and animal vocalizations. Qwen, Kimi-Audio, and
Step-Audio-2-mini receive the same test audio, with 100 examples per class.
We evaluate each target in its clean form and after mixing with
interference at $-10$ dB. The PCA memories use
$N\in\{20,50,100\}$ clean examples per class.

All models receive the same twenty candidate labels for constrained
classification. Without these labels, we count a free-form description as
correct only when it unambiguously identifies the target category. The
retrieval protocol instead scores the representations against the
separately constructed clean reference gallery. Table~\ref{tab:twenty_class_main}
reports the macro-average accuracy across all twenty classes.

\begin{table}[t]
\centering
\caption{Macro-average accuracy (\%) over twenty sound classes. ``Con.''
denotes constrained classification, ``Free'' denotes free-form
classification, and ``Ret.'' denotes prompt-free token retrieval.}
\label{tab:twenty_class_main}
\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{llccccc}
\toprule
Model & Protocol & Clean & $-10$ dB Mix & PCA-20 & PCA-50 & PCA-100 \\
\midrule
Qwen
& Con.  & 66.90 & 9.60 & 47.20 & 48.95 & 49.20 \\
& Free  & 32.05 & 4.80 & 26.25 & 26.20 & 27.60 \\
& Ret.  & 87.90 & 8.25 & 86.75 & 86.75 & 86.10 \\
\midrule
Kimi-Audio
& Con.  & 58.20 & 8.30 & 59.70 & 58.25 & 57.60 \\
& Free  & 38.45 & 4.90 & 45.80 & 44.25 & 43.30 \\
& Ret.  & 80.40 & 11.25 & 75.60 & 72.60 & 74.30 \\
\midrule
Step-Audio-2-mini
& Con.  & 72.50 & 10.25 & 42.05 & 45.80 & 44.80 \\
& Free  & 57.30 & 7.15 & 42.45 & 42.95 & 44.65 \\
& Ret.  & 88.95 & 10.45 & 78.50 & 83.65 & 82.50 \\
\bottomrule
\end{tabular}
\end{table}

Target-class readout is lower on mixed than on clean audio for every model
and evaluation protocol. In prompt-free retrieval, Qwen accuracy falls from
87.90\% to 8.25\%. Supplying the target memory raises it to 86.75\% at the
best enhanced setting. The same pattern appears in Kimi-Audio, where the
clean and mixed accuracies are 80.40\% and 11.25\%, and enhancement reaches
75.60\%. For Step-Audio-2-mini, these values are 88.95\% and 10.45\%, with
enhancement reaching 83.65\%. Across all three models, the supplied memory
brings retrieval accuracy closer to the clean baseline.

This change in the representations also carries through to language output.
For Kimi-Audio, constrained classification improves from 8.30\% on mixed
audio to 59.70\% with PCA-20, while free-form classification improves from
4.90\% to 45.80\%. Qwen reaches 49.20\% constrained accuracy and 27.60\%
free-form accuracy at PCA-100. Step-Audio-2-mini reaches 45.80\% constrained accuracy
at PCA-50 and 44.65\% free-form accuracy at PCA-100.

The enhanced retrieval scores remain higher than those obtained through
language output. This is consistent with PCA acting directly on the
similarity between representations, while generating an answer requires a
further step through the language model. The preferred memory size also
differs across models. Qwen changes little across the three values of $N$,
whereas Kimi-Audio performs best at $N=20$. Step-Audio-2-mini reaches its
best retrieval score at $N=50$. More clean examples therefore do not
guarantee better readout.

\paragraph{Speech content fidelity under token-wise control.}
We next examine whether the optional token-wise gate in
Section~\ref{sec:memory_gate} limits the loss of instance-specific speech
content caused by a fixed memory correction. The category memory is constructed
from $N=500$ clean speech examples, and the calibrated reconstruction uses
$k=8$ and $\alpha=0.7$. We train only the gate for four epochs, using a learning
rate of $10^{-3}$ and $\lambda_{\mathrm{text}}=1$; the PCA memory and the ALLM
remain frozen throughout.

To separate hyperparameter selection from final evaluation, we partition the
100-example validation set into 80 training and 20 selection mixtures with
seed 20260919. We sweep
$\lambda_{\mathrm{tok}}\in\{0.0,0.1,\ldots,1.0\}$ on the selection split,
choose the value with the lowest selection WER (breaking ties toward the
smaller value), retrain the gate on all 100 validation examples, and evaluate
the selected setting once on the held-out 100-example test set. The test set is
not used for training or hyperparameter selection in this protocol.

\begin{table}[t]
\centering
\caption{Validation selection and held-out evaluation of the optional
token-wise gate. S/D/I denotes substitution, deletion, and insertion counts.
The validation selection split contains 175 reference words; the final test
set contains 880 reference words.}
\label{tab:voicefilter_gate}
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{lcccc}
\toprule
Stage & $\lambda_{\mathrm{tok}}$ & Examples & S / D / I & WER (\%) \\
\midrule
Selection split & 0.1 & 20 & 23 / 10 / 3 & 20.57 \\
Held-out test & 0.1 & 100 & 63 / 48 / 19 & 14.77 \\
\bottomrule
\end{tabular}
\end{table}

The independent selection split chooses $\lambda_{\mathrm{tok}}=0.1$ with a
WER of 20.57\%. After retraining on all validation examples, the selected gate
obtains 14.77\% WER on the held-out test set. Because the test result is
reported only after the loss weight has been fixed, it provides a confirmatory
measurement of speech-content fidelity rather than another point in the
hyperparameter sweep.

\subsection{Analysis and Discussion}
\label{sec:analysis}
\paragraph{Recovery efficiency.}
To quantify how much performance is recovered after enhancement, we define
the recovery ratio as
\[
R =
\frac{\mathrm{Acc}_{\mathrm{PCA}}-\mathrm{Acc}_{\mathrm{mixed}}}
{\mathrm{Acc}_{\mathrm{clean}}-\mathrm{Acc}_{\mathrm{mixed}}}.
\]
Under prompt-free retrieval, the best PCA setting recovers 98.6\% of the
gap between clean and mixed performance for Qwen. The corresponding ratios
are 93.1\% for Kimi-Audio and 93.2\% for Step-Audio-2-mini. These similar
values describe the change in readout when the target memory is supplied.
The enhanced and unenhanced conditions receive different target
information, so the ratio does not quantify recovery of acoustic
information specific to the current instance.

For Kimi-Audio, the best constrained and free-form results exceed the
corresponding clean baselines, producing recovery ratios above 100\%.
The supplied memory introduces information about the known target category
that the clean baseline does not receive. Exceeding that baseline therefore
does not establish that the enhanced representation is intrinsically better
than a clean representation.

\paragraph{Representation recovery versus semantic prediction.}
The difference between retrieval and language output helps interpret these
gains. Prompt-free retrieval measures whether the enhanced representation
becomes closer to clean examples of the correct class. Constrained and
free-form classification additionally depend on the model's ability to
generate a description or select a label. These additional steps can affect
how a change in the audio representation appears in the final answer.

The guitar ablation illustrates this distinction. PCA reduces its token MSE
by more than 42\%, but its classification accuracy remains close to zero.
Similarly, direct projection onto the clean guitar subspace achieves 71\%
accuracy in the projection diagnostic, whereas routing consistency remains
only 34\%. Thus, reducing representation distance does not necessarily
restore the semantic decision path required for correct classification.

\paragraph{Class and model dependence.}
The early ablations also show why a single configuration may not suit every
class. Piano accuracy remains near 100\%, while the gains for dog
vocalization depend on the parameters and guitar remains difficult. LoRA
adaptation improves dog recognition but degrades guitar recognition. In the
twenty-class study, the preferred number of clean examples also varies
across models and evaluation protocols. These observations motivate choosing
the memory size for each class, alongside its rank and enhancement strength.

\paragraph{Limitations.}
The current experiments use the ground-truth category to select the memory.
They characterize how this supplied prior affects target readout, while
automatic target discovery in an unknown mixture remains open. An automatic
memory selector would address that part of the problem. The twenty-class
evaluation is also restricted to $-10$ dB mixtures and three memory sizes.
Evaluation at other signal-to-noise ratios and with different interference
would help establish the range of the effect. Repeated data samplings and
random seeds are needed to measure its variability.


==> Papers/Papers/5_Conclusions.tex <==
\section{Conclusions}
